The Stochastic Matching Problem: Beating Half with a Non-Adaptive Algorithm

In the stochastic matching problem, we are given a general (not necessarily bipartite) graph $G(V,E)$, where each edge in $E$ is realized with some constant probability $p > 0$ and the goal is to compute a bounded-degree (bounded by a function depending only on $p$) subgraph $H$ of $G$ such that the expected maximum matching size in $H$ is close to the expected maximum matching size in $G$. The algorithms in this setting are considered non-adaptive as they have to choose the subgraph $H$ without knowing any information about the set of realized edges in $G$. Originally motivated by an application to kidney exchange, the stochastic matching problem and its variants have received significant attention in recent years. The state-of-the-art non-adaptive algorithms for stochastic matching achieve an approximation ratio of $\frac{1}{2}-\epsilon$ for any $\epsilon > 0$, naturally raising the question that if $1/2$ is the limit of what can be achieved with a non-adaptive algorithm. In this work, we resolve this question by presenting the first algorithm for stochastic matching with an approximation guarantee that is strictly better than $1/2$: the algorithm computes a subgraph $H$ of $G$ with the maximum degree $O(\frac{\log{(1/ p)}}{p})$ such that the ratio of expected size of a maximum matching in realizations of $H$ and $G$ is at least $1/2+\delta_0$ for some absolute constant $\delta_0 > 0$. The degree bound on $H$ achieved by our algorithm is essentially the best possible (up to an $O(\log{(1/p)})$ factor) for any constant factor approximation algorithm, since an $\Omega(\frac{1}{p})$ degree in $H$ is necessary for a vertex to acquire at least one incident edge in a realization.

==> app-conc.tex <==
\section{Open Problems}\label{app:conc}

We presented the first non-adaptive algorithm with an approximation ratio that is strictly better than half for stochastic matching. In
particular, we showed that there exists an algorithm that given any graph $G$, computes a subgraph $H$ of $G$ with maximum degree $O(\frac{\log{(1/p)}}{p})$ such
that the ratio of expected size of a maximum matching in realizations of $H$ and $G$ is at least $0.52$ when $p$ is sufficiently small, and
$0.5+\delta_0$ (for an absolute constant $\delta_0 > 0$) for any values of $ 0 < p < 1$.

A main open problem remained by our work is to determine the best approximation ratio that a non-adaptive algorithm for stochastic matching can achieve. 
In particular, can non-adaptive algorithms match the performance of adaptive algorithms
by achieving a $(1-\eps)$-approximation for any $\eps > 0$? 




==> b-limitation.tex <==
\section{The Optimality of the $b$-Matching Lemma}

In this section, we establish that our $b$-matching lemma is essentially optimal in the sense that it is impossible to find a $b$-matching
with at least $b\cdot \opt(G)$ edge for $b$ much larger than $1/p$. In particular, we show that,

\begin{claim}\label{clm:b-match-opt} 
  For any constant $0 < p < 1$, there exist bipartite graphs $G$ where $G_p$ has a matching of size $n-o(n)$ in expectation, and for any
  $b > {2 \over p}$, there is no $b$-matching in $G$ with (at least) $b\cdot 0.99n$ edges; here $n$ is the number of
  vertices on each side of $G$.
\end{claim}
\begin{proof}
  Consider bipartite graphs $G(L,R,E)$ where the vertices in $L$ consists of two disjoint sets $L_1$ and $L_2$ with $\card{L_1} = N$ and
  $\card{L_2} = N/e$, for the parameter $N = {n \over (1 + 1/e)}$. Similarly, $R$ contains two sets $R_1$ and $R_2$ with $\card{R_1} = N$
  and $\card{R_2} = N/e$.
  
  The edges in $G$ consists of two parts. First, there is a complete bipartite graph between $L_1$ and $R_2$, and a complete bipartite graph
  between $L_2$ and $R_1$. Second, there is a sparse graph between $L_1$ and $R_2$ defined through the following random process: each edge
  between $L_1$ and $R_1$ is chosen w.p. ${1 \over pN}$, independent of each other.

  In the following, we show that for a graph $G$ created through the above process, w.p. $1 - o(1)$, $G_p$ has a matching of size $n-o(n)$
  in expectation, and w.p. $1 - o(1)$, there is no $b$-matching in $G$ with $b\cdot 0.99n$ edges, for $b > {2 \over p}$. Hence, by applying a
  union bound, the above process find a graph with both properties w.p.  $1 - o(1)$, proving the claim.
  
  To see that $G_p$ has a matching of size $n-o(n)$ in expectation, we realize the edges in $G$ in two steps: first realize the edges
  between $L_1$ and $R_1$, and then the other edges (i.e., the two complete graphs between $L_1, R_2$ and between $L_2, R_1$,
  respectively). For the subgraph between $L_1$ and $R_1$, notice that each edge between $L_1$ and $R_1$ is realized w.p.
  ${1 \over pN} \cdot p = {1 \over N}$ (chosen w.p. ${1 \over pN}$ in the above process and realize w.p. $p$). Since
  $\card{L_1} = \card{R_1} = N$, the subgraph between $L_1$ and $R_1$ is a random bipartite graph with $N$ vertices on each side where each
  edge is chosen w.p. $1/N$, independently. Therefore, by~\cite{bollobas1998random}, w.p. $1-o(1)$, there is a matching of size $(1 - 1/e)N$
  between $L_1$ and $R_1$. Now for the remaining $N/e$ unmatched vertices in $L_1$ (resp. in $R_1$), since there is a complete graph between
  $L_1$ and $R_2$ (resp. $R_1$ and $L_2$), w.p.  $1 - o(1)$, a perfect matching realizes between the unmatched vertex in $L_1$ and $R_2$
  (resp. between $R_1$ and $L_2$). The total matching size is $(1 - 1/e)N + N/e + N/e = (1 + 1/e)N = n$, and the expected maximum matching
  size in $G_p$ is at least $(1 - o(1)) n + o(1) \cdot 0 = n - o(n)$.

  It remains to show that w.p. $1 - o(1)$, $G$ has no $b$-matching with $b\cdot 0.99n$ edges for $b>{2 \over p}$. For any $b$-matching in $G$,
  the number of edges incident on $L_2$ and $R_2$ is at most $b \cdot (\card{L_2} + \card{R_2}) = 2 b N/e$. The remaining edges of this
  $b$-matching must be between $L_1$ and $R_1$. Each edge between $L_1$ and $R_2$ is chosen w.p. ${1 \over pN}$, and there are $N^2$
  possible edges between $L_1$ and $R_1$. By Chernoff bound, w.p. $1 - o(1)$, the number of realized edges between $L_1$ and $R_1$ is at
  most $(1 +\eps_0) {N \over p}$ (for a constant $\eps_0$ to be fixed later). Therefore, the total number of edges of any $b$-matching in
  $G$ is at most
  \begin{align*}
    2 b N/e + (1 + \eps_0){N \over p} &= b\cdot n - b(1 - 1/e)N + (1 + \eps_0) {N \over p}\tag{$(1 + 1/e)N = n$}\\
    & < b\cdot n - \paren{(1 - 1/e) - {1 + \eps_0 \over 2}}bN  \tag{$b > 2/p$ and hence $1/p < b/2$}\\
    & = b\cdot 0.99 n \tag{fix $\eps_0$ s.t., $1 - {1 \over e} - {1 + \eps_0 \over 2} = 0.01 (1 + {1\over e})$ ($\eps_0 \approx 0.24$)}
    \end{align*}
\end{proof}

==> missing.tex <==
\section*{Omitted Proofs}\label{app:missing}

\subsection{Proof of Proposition~\ref{prop:upper-exp}}\label{app:upper-exp}
\begin{proposition*}
  Let $f(x) := {1 - e^{-x} \over x}$. Then, for any $c$, and any $x \in [0, c]$, $e^{-x} \le 1 - f(c) \cdot x$.
\end{proposition*}
\begin{proof}
	We first have $f(x)$ is \emph{monotone decreasing}, since, 
	\begin{align*}
		\frac{d f}{d x} = \frac{e^{-x} \cdot x - 1+e^{-x}}{x^2} = \frac{(x+1)\cdot e^{-x} - 1}{x^2} \leq \frac{e^{x}\cdot e^{-x} - 1}{x^2} = 0 
	\end{align*}
	where we used the inequality $(1+x) \leq e^{x}$. 
	
  Consequently, since $x \le c$, 
  \begin{align*}
    f(c) \le f(x) = {1 - e^{-x} \over x}
  \end{align*}
  which implies $e^{-x} \le 1 - f(c) \cdot x$.
\end{proof}


\subsection{Proof of Proposition~\ref{prop:upper-exp-2}}\label{app:upper-exp-2}
\begin{proposition*}
  For any $x \in (0,1]$, $(1-x)^{{1\over x}} \ge {1 - x \over e}$.
\end{proposition*}
\begin{proof}
  We first exam the equivalent conditions for the target inequality.
  \begin{align*}
    &                             &(1-x)^{{1\over x}} \ge {1 - x \over e} \\ 
    &\Longleftrightarrow &     (1-x)^{{1\over x} - 1} \ge {1 \over e} \\
    &\Longleftrightarrow &     ({1\over x} - 1)\log(1-x) \ge -1 \tag{Take natural log  for both sides.}
  \end{align*}
  Now, since $\log(1 - x) \ge -x - {x^2 \over 2} - {x^3 \over 2}$ when $x \in (0,0.43]$. We have 
  \begin{align*}
    ({1\over x} - 1)\log(1-x) &\ge ({1\over x} - 1) (-x - {x^2 \over 2} - {x^3 \over 2}) \tag{since $({1\over x} - 1) > 0$} \\
    & = -1 - {x \over 2} - {x^2 \over 2} + x + {x^2 \over 2} + {x^3 \over 2} \\
    & = - 1 + {x \over 2} + {x^3 \over 2} \\
    & \ge -1
  \end{align*}
  which completes the proof.
\end{proof}


\subsection{Proof of Claim~\ref{clm:small-L}}\label{app:small-L}
\begin{claim*}
	Fix $0 < \eps < \delta < 1$. Let $G(V,E)$ be a graph, $X$ be any arbitrary subset of $E$, and $(M_1,\ldots,M_R) = \basicalg(G(V,E\setminus X),\eps)$. 
	Define $E_{MC} = M_1 \cup \ldots \cup M_R$. 	If $\card{M_R} \leq \paren{\frac{1}{2}-\delta} \OPT$, then the expected maximum matching size in a realization
	of $G(V, X \cup E_{MC})$ is at least $\paren{\frac{1}{2} + \delta - \eps} \OPT$. 
\end{claim*}

\begin{proof}
For each realization of $G_p$, we fix one maximum matching. Now the expected matching size in $G_p$
  can be written as
  \begin{align*}
    {\OPT} = \sum_M\prob{\text{$M$ is the fixed maximum matching in $G_p$}} \cdot \card{M}
  \end{align*}
  By property~(2) of \basicalg in Lemma~\ref{lem:basic-alg}, the maximum matching size in the graph $G(V,E \setminus (X \cup E_{MC}))$ is at most $(1+\eps)\card{M_R}$. 
  Therefore, for any matching $M$, at most $(1+\eps)\card{M_R}$ edges of $M$ is in $E \setminus (X \cup E_{MC})$, and hence at least $\card{M} - (1+\eps)L$ edges
  of $M$ is in $X \cup E_{MC}$. This implies that if all edges in $M$ are
  realized, a matching of size at least $\card{M} - (1+\eps)\card{M_R}$ is realized in $Q$. Let $\ALG$ be the expected maximum matching size in $G(V,X \cup E_{MC})$; we have,  
  \begin{align*}
  \ALG &\ge \sum_M\prob{\text{$M$ is the fixed maximum matching in $G_p$}} (\card{M} - (1+\eps)\card{M_R})\\
                  &={\OPT} - (1+\eps)\card{M_R}
  \end{align*}
  Since $\card{M_R} \le (1/2 - \delta){\OPT}$, we have, 
  \[ \ALG \ge {\OPT} - (1+\eps)\cdot(1/2 - \delta) \cdot {\OPT} \geq (1/2 + \delta - \eps) \cdot {\OPT}\]
  which concludes the proof.
\end{proof}

\subsection{Proof of Lemma~\ref{lem:outside-edges}}\label{app:outside-edges}
\begin{lemma*}
  Let $B$ be a $\floor{\frac{1}{p}}$-matching with $\paren{\floor{\frac{1}{p}}\cdot N}$ edges; then, $\EX{\mu(B_p)} \geq (1-3p) \cdot {\frac{N}{3}}$.
\end{lemma*}

\begin{proof}
	We first partition the edges of $B$ into a collection of matchings. Since the degree of each vertex in $G(V,B)$ is at most $\floor{\frac{1}{p}}$, by Vizing's Theorem~\cite{Vizing64}, we can color
	the edges in $G(V,B)$ with $\floor{\frac{1}{p}}+1$ colors such that no two edges with the same color are incident on a vertex.
	This ensures that $B$ can be decomposed into $R = \floor{\frac{1}{p}}+1$ matchings
	$M_1,\ldots,M_R$. 

	Next, we define the following process. Define $M^{(0)} = \emptyset$; for $i = 1$ to $R$ rounds, let $M^{(i)}$ be a maximal matching
        obtained by adding to $M^{(i-1)}$ the set of realized edges in $M_i$ that are not incident on vertices in $M^{(i-1)}$. Define
        $M := M^{(R)}$. 
        
        We argue that $\Ex{\card{M}} \geq (1-3p) \cdot {\frac{N}{3}}$. To do this, we need the following notation. Define $Y_i$ as a random variable denoting 
	the \emph{set of edges} in $M_i$ that are \emph{not} incident on any vertex of matching $M^{(i-1)}$. Note that $Y_i$ depends only on the realization of edges in $M_1,\ldots,M_{i-1}$ and is \emph{independent} of 
	the realization of $M_i$. Moreover, define $X_i$ as a random variable indicating the \emph{number of edges} in (a realization of )$Y_i$ that are added to $M^{(i-1)}$ (after updating by edges in $M_i$). We first have, 
	\begin{align*}
		\card{Y_i} \geq \card{M_i} - 2 \card{M^{(i-1)}}
	\end{align*}
	since any edge in $M^{(i-1)}$ can be incident on at most two vertices of $M_i$. Moreover, conditioned on any valuation
	for $Y_i$, we have $\Ex{X_i} = p \cdot \card{Y_i}$ since each edge in $M_i$ is realized w.p. $p$, independent 
	of the choice of $Y_i$. Consequently, 
	\begin{align*}
		\Ex{X_i} = p \cdot \Ex{Y_i} \geq p \cdot \paren{\card{M_i} - 2\EX{\card{M^{(i-1)}}}}
	\end{align*}
	We again stress that the expectation for $X_i$ is taken over the choice of edges in $M_i$, while the expectation for $Y_i$ (and $M^{(i-1)}$) is taken over the choice of edges in $M_1,\ldots,M_{i-1}$. 
	We now have, 
	\begin{align*}
		\Ex{\card{M}} &= \sum_{i=1}^R \Ex{X_i} \geq \sum_{i=1}^{R} p \cdot \paren{\card{M_i} - 2\EX{\card{M^{(i-1)}}}} \\
		&\geq p \cdot \paren{\sum_{i=1}^{R} \card{M_i} - 2 \sum_{i=1}^{R} \Ex{\card{M}}} \tag{$\Ex{\card{M}} \geq \EX{\card{M^{(i-1)}}}$} \\
		&\geq p \cdot \paren{\floor{\frac{1}{p}} \cdot N - 2 \paren{\floor{\frac{1}{p}}+1} \cdot \Ex{\card{M}}} \tag{$R = \floor{\frac{1}{p}}+1$}
	\end{align*} 
	This implies that 
	\begin{align*}
		\Ex{\card{M}} \geq (1-3p) \cdot \frac{N}{3}
	\end{align*}
	which concludes the proof.
\end{proof}
